Multiple Set Matching and Pre-Filtering with Bloom Multifilters

Bloom filter is a space-efficient probabilistic data structure for checking elements' membership in a set. Given multiple sets, however, a standard Bloom filter is not sufficient when looking for the items to which an element or a set of input elements belong to. In this article, we solve multiple set matching problem by proposing two efficient Bloom Multifilters called Bloom Matrix and Bloom Vector. Both of them are space efficient and answer queries with a set of identifiers for multiple set matching problems. We show that the space efficiency can be optimized further according to the distribution of labels among multiple sets: Uniform and Zipf. While both of them are space efficient, Bloom Vector can efficiently exploit Zipf distribution of data for further space reduction. Our results also highlight that basic ADD and LOOKUP operations on Bloom Matrix are faster than on Bloom Vector. However, Bloom Matrix does not meet the theoretical false positive rate of less than $10^{-2}$ for LOOKUP operations if the represented data or the labels are not uniformly distributed among the multiple sets. Consequently, we introduce \textit{Bloom Test} which uses Bloom Matrix as the pre-filter structure to determine which structure is suitable for improved performance with an arbitrary input dataset.

==> sections/distributed_bmfs.tex <==
\section{Distributed Bloom Vectors} \label{distributed_bmfs}

%\begin{figure}
%    \centering
%    \includegraphics[width=\linewidth]{figures/distributed_bmf}
%    \caption{Distributed Bloom Multifilters. Data files are located in a distributed environment in multiple computing nodes or data nodes (slaves in the figure). Each computing node creates a local BMF and keeps it in memory. For $\LOOKUP$ operations, the master broadcasts the query and merges the results from the slaves. In the case of a union operation, the master constructs the final BMF structure by reducing the BMFs from the cluster nodes. }
%    \label{fig:par_union}
%\end{figure}

\begin{figure}
	\begin{verbatim}

/*(1) construct BMF Objects*/
val bloomRDD = docs.mapPartitions(docs => {
 //dc => Array[String, Array[String]]
 //fprate => false positive rate
 val dc = doc.toArray
 val bv = new BloomVector(dc,fprate)
 // k = number of hashes
 // m = number of bits
 //val bv = new BloomVector(dc,m,k)
 Iterator.apply(bv)}).cache
 
(2)/* query labels in BMF objects*/ 
val query = sc.broadcast("magic")
val lookupDocs =  bloomRDD.map(bv => {
  val operator = "and"
  val docs= bv.lookup(query.value,operator)
  (docs)
}).reduce( (f1, f2) => (f1 ++ f2))
	\end{verbatim}
	\caption{Distributed operations on Bloom Vector structures in Spark big data framework}
	\label{fig:sparkapis}
\end{figure}

%In the earlier section, we demonstrated that concurrent Bloom Filter operations can improve the time efficiency of $\ADD$ and $\LOOKUP$ operations. However, such parallelism may not be suitable for large volumes of encoded data. In this section, we discuss distributed operations on BMF objects and their performance, through practical implementation and measurements.

%Distributed big data frameworks, such as Spark~\cite{ZCD12}, are suitable for dealing with large data volumes, such as the Wikipedia corpus. Such frameworks work in a cluster environment in which the data is distributed among the computing nodes in the cluster. A master node coordinates the distribution of the data and the computation. Each computing node can operate on raw data to compute their own BMF.
In this section, we demonstrate how Bloom Vector and the operations can be distributed with Spark. We use the Wikipedia corpus. The corpus contains an \textsf{XML} file with a size of 66 GB, consisting of 17 million pages. Each document is represented with its page ID and a bag of distinct words.   %It is very likely that the number of unique words varies drastically from page to page, and a significant number of pages have only a few words. In Figure~\ref{fig:memovh}, we have already shown that overhead can be quite significant for the BMFs with such skewed distribution, except for the OBV. Therefore, we chose the OBV to represent the Wikipedia corpus.



%Whenever the master node receives a request, $\ADD$ or $\LOOKUP$, it broadcasts the query to the computing nodes. Additionally, the master can perform a reduce operation on the data structures collected from the computing nodes to a single data structure. %The rationale is that, since the structures are compact, the master node can hold the merged BMF in memory. Therefore, it can use the nodes to create BMFs from local data and merge them into a single BMF. Furthermore, the lookup time may reduce, as the overhead for networking is reduced.



%\subsection{Dataset Pre-processing and Distributed MBFs} 

%The corpus contains an \textsf{XML} file with a size of 66 GB, consisting of 17 million pages. Each page contains a page ID and text, along with a number of other attributes. We have cleaned the corpus in two steps with Spark. First, we loaded the \textsf{XML} file with Spark and separated ID and the text attributes. In the second step, the text field is cleaned by filtering out different non-letter characters, other stop words, and later converted to lowercase.  Therefore, each document is represented with its page ID and a bag of distinct words. We obtained 1.21 Billion words (labels) from 17 million pages. The final dataset has a size of 11GB split over 360 partitions. Each partition contains a list of documents, represented by an ID and its bag of words as comma separated values.
 We have cleaned the corpus in two steps using Spark. First, we loaded the \textsf{XML} file with Spark and separated ID and the text attributes. In the second step, the text field is cleaned by filtering out different non-letter characters, other stop words, and later converted to lowercase.  Therefore, each document is represented with its page ID and a bag of distinct words.  %Since spark uses Resilient Distributed DataSet (RDD) semantic for memory-based distributed data abstraction, it is possible to cache the RDDs in memory.
After pre-processing, we obtained 1.21 Billion words (labels) from 17 million pages, i.e., $|E|$=17$\times10^6$. The final dataset had a size of 11GB split over 360 partitions. The preprocessing and all other measurements presented in this section were achieved with a computer having 96 cores and 3TB RAM.  The Spark cluster was configured with 90 cores, 45 executors, and 800 GB RAM.


\begin{figure}
    \centering
    \subfloat[Size of BVs\label{bvspark-s}] {\includegraphics[width=0.48\linewidth]{figures/sparkobvspace.eps}}
\subfloat[Time to add labels\label{bvspark-t}]     {\includegraphics[width=0.48\linewidth]{figures/addtimeSbv.eps}}
    \caption{The size of the BV objects with different FP rates and the average time to add a single word or all the unique words in a documents to the OBVs in a Spark RDD.}
    \label{fig:spark_bvadd}
\end{figure}


\subsection{Add}

%We implemented the APIs based on the Scala class representation of the basic BMFs. Figure~\ref{fig:sparkapis} shows how Spark RDDs of BMF structures can be constructed from partitions of the Wikipedia articles. The basic APIs accept as inputs the number of bits and the number of hash functions. If the desired structure is BM, the APIs also provide a parameter to specify whether such structure should be the sparse version or not. It is also possible to construct BMF objects given a specific FP rate.

The $\ADD$ operation is applied at the very beginning while constructing a Bloom Vector object for the very first time. In this case, a local BV object is created by loading the data contained in a partition.   %This is necessary to ensure that the words of a page are not spread among multiple partitions. This further ensures a lower false FP rate. Both operations are shown in ~\ref{fig:sparkapis}. 
In the end, we obtained an RDD of 360 BVs. The construction of \textsf{bloomRDD}  of BV is  shown in ~\ref{fig:sparkapis}.  We constructed a set of 360 BVs with different FPs. Adding words to an already constructed  Bloom Vector, however, requires the master to broadcast the document ID together with the word. The executors check whether a particular page exists in a partition or not.

Figure~\ref{bvspark-s} shows the total size of 360 BV objects  with different FP rates. Compared to the actual size of the dataset, we notice that total size of the BV objects increases, as the FP rate decreases. This is because the size of each Bloom Filter increases as the FP rate decreases. The maximum reduction is 76\% and achieved when the FP rate is 0.1. Even with the FP rate of $10^{-6}$, the total size of the BVs is lower than 6 GB.

The figure also shows the average time required to add a single label and all the labels in a document to the BV objects. We can see that the $\ADD$ operation requires more time as the FP decreases.



%\subsection{Union}

%\begin{figure}
%	\begin{verbatim}
%/* merge BMFs from the computing nodes*/
%val bmfMerge =  bloomRDD.reduce(_ union _)
%	\end{verbatim}
%	\caption{Distributed operations on BMF structures in Spark big data framework}
%	\label{fig:mergeunion}
%\end{figure}

%With the Union operation, it is important that all the BMFs stored in slave nodes have compatible parameters. This is because, if each slave creates an optimal BMF for its assigned partition, it is very likely that the master will not be able to merge them, or that the \ac{FP} rate will be higher than expected. Therefore, all the slave or the computing nodes in the cluster must have OBV objects with similar parameters, i.e. $k$. Since the words of a document are not spread over multiple slaves, the reduce operation is simplified to a concatenation of the different BMF objects. In case of documents split among different partitions, it is required to merge the rows that represent the same documents while merging.

%Figure~\ref{fig:mergeunion} shows the Spark code snippet for the BV merge operation. This is implemented as the reduce function with the union operator that merges all the OBVs into a single OBV object at the master.




\subsection{Lookup}

Figure~\ref{fig:sparkapis} shows an example $\LOOKUP$ operation implementation with Spark. The operation is implemented so that the master node broadcasts the query word to the computing nodes or slaves, and the nodes respond with the corresponding page IDs from the local BMF objects. The master finally merges all the results from the slaves. The $\LOOKUP$ queries were executed on the cached RDD of BV objects, as shown in Figure~\ref{fig:sparkapis}.

We implemented two different $\LOOKUP$ operations for multiple queries; $\mathbf{\lor}$ (or) and $\mathbf{\land}$ (and). Figure~\ref{fig:sparklookup} compares the lookup time while querying one thousand words to the distributed OBVs with different FP rates. We notice that lookup time for OR queries decreases until the FP rate decreases to 0.09 and then increases exponentially as the FP rate further decreases. The average lookup time for a single label is a few hundred milliseconds (234 ms) even when the FP rate is the lowest $10^{-6}$. The behaviour is clearer for $\LOOKUP$ operations with 10 words. The lookup time slowly decreases until we have a $10^{-3}$ FP rate, and then increases again. The average lookup time of a label reduces to 4 ms.
 
The lookup time also behaves similarly with the AND query. In this case, the total lookup time increases from 20 s to a maximum of 192 s for the query with one thousand words.
Such AND query is impractical, therefore, we also queried for 10 words, the total lookup time reduces to 1.2 seconds when the FP rate is $10^{-3}$. However, the trend is similar to all the queries. The obvious reason is that the number of hash functions increases as the FP rate decreases. Therefore, it takes a longer time to compute the results. The results are similar to those presented in Section~\ref{experimental_results}.

We also investigate the performance of a lookup operation using Spark APIs, by implementing optimized AND and OR operations. Similarly to the approach described above, the master broadcasts the query. The lookup operations are called inside a filter operation on a cached \texttt{RDD[(String, List[String])]} structure for checking the membership and association. We measured that Spark took 67 and 61 seconds respectively for AND and OR queries with 1000 words. In case of 10 words, Spark with OBV took the lowest 1.2 and 2.2 seconds for AND and OR operations respectively, whereas Spark without OBV took respectively 2 and 3.1 seconds. In both cases, Spark with OBV is faster than standalone Spark only when the FP rate is higher than 0.001.


\begin{figure}
    \centering
     \includegraphics[width=1.0\linewidth]{figures/sparklookup.eps}
    \caption{Query response time for lookup  1000 words with $\land$ and $\lor$ operations. The response of these queries are the Wikipedia page IDs.}
    \label{fig:sparklookup}
\end{figure}

%\begin{figure}
%    \centering
%     \includegraphics[width=1.0\linewidth]{figures/cardinquery.eps}
%    \caption{Average response time for the cardinality estimation queries on top of the complete dataset with respect to  FP rates.}
%    \label{fig:basicqrestime}
%\end{figure}

%\subsection{Cardinality Queries}

%We also investigate the performance of Spark with and without BMFs for checking the cardinality on the total number of documents and the approximate number of labels. As mentioned earlier, we implemented BMF classes to answer the total number of elements $|E|$ and the approximate number of labels $|L|$. The line plots in Figure~\ref{fig:basicqrestime} show that counting the total number of pages takes a few hundred milliseconds for different FP rates. Similarly, counting the approximate number of labels of the corpus takes 1 to maximum 2 seconds. In both cases, the computing time increases slowly as the FP rate increases. On the other hand, with Spark APIs, these queries take on an average 1.6 and 2.2 seconds, respectively.


\subsection{Discussion}

Dealing with a large volume of data is challenging without distributed computing platforms. In this section, we have demonstrated how to construct BMF structures with Spark from raw datasets. These structures are very space and time efficient to construct and enable the platform to answer some basic queries faster. 

Although in a Spark cluster environment, the master is expected to have a significant amount of memory. Therefore, it is reasonable to expect that the master would be able to keep the merged BMF in the memory. Alternatively, it is also possible for the master to collect all the BMFs from the slave nodes and keep them stored inside an array. It is intuitive that such approach may further speed up the $\LOOKUP$ operation by avoiding network latency. However, with a huge amount of encoded data, the master must have a certain degree of parallelism capability in order to improve the performance.

Finally, we have shown that the BMF objects are so small that the slave nodes in a cluster can keep multiple variations of them in memory at a time. The applications can iterate back and forth among them according to the query requirement. For example, as we have already seen in this section, the performance of $\LOOKUP$ operations depends on the size of the query as well. Therefore, it is possible to keep OBVs with different FP rates in memory and select the OBV of a particular FP rate based on the number of queries. For example, when the size of the query is relatively small, the system can use OBVs with lower FP rates. And for large queries, the system can rely on OBVs with higher FP rates.


==> tikzfig/multiunilookup.tex <==
\nextgroupplot[
        legend cell align=left,
        legend style={at={(0.5,1.13)},anchor=west,draw=none,fill=none},
        legend columns=5,
        title=Uniform,
        %legend pos = north east,
        xmode = log,
        ymode = log,
		ylabel= Avg. Lookup Time (ms),
        ylabel style = {yshift=-1ex},
		%axis x line*=bottom,% only show the bottom x axis line, without an arrow tip
    	ymin=0.00001, ymax=0.07,% range for the x axis
        %xmin = 1, xmax = 11,
        %x dir=reverse,
    	xlabel = \# Lookup Labels       %yticklabels={,,},
        %xticklabels={1,10,100,1000},
        %yticklabels = {0.00,0.01,0.02,0.03,...,0.04,0.05},
		]         
\addplot+[mark=none,draw=black, thick] table {
1 0.00001461
10 0.00020852
100 0.00029274
1000 0.00106649
};
\addplot+[mark=none,draw=black, dashed] table { 
1	0.00004315
10	0.00028716
100	0.00121272
1000	0.00869999
};

\addplot+[mark=none,draw=black, densely dotted] table { 
1 0.00018569
10 0.00069226
100 0.00444938
1000 0.02298746
};


\legend{BM, SBM, BV};


